Linguistic Characterization of Divisive Topics Online: Case Studies on Contentiousness in Abortion, Climate Change, and Gun Control

As public discourse continues to move and grow online, conversations about divisive topics on social media platforms have also increased. These divisive topics prompt both contentious and non-contentious conversations. Although what distinguishes these conversations, often framed as what makes these conversations contentious, is known in broad strokes, much less is known about the linguistic signature of these conversations. Prior work has shown that contentious content and structure can be a predictor for this task, however, most of them have been focused on conversation in general, very specific events, or complex structural analysis. Additionally, many models used in prior work have lacked interpret-ability, a key factor in online moderation. Our work fills these gaps by focusing on conversations from highly divisive topics (abortion, climate change, and gun control), operationalizing a set of novel linguistic and conversational characteristics and user factors, and incorporating them to build interpretable models. We demonstrate that such characteristics can largely improve the performance of prediction on this task, and also enable nuanced interpretability. Our case studies on these three contentious topics suggest that certain generic linguistic characteristics are highly correlated with contentiousness in conversations while others demonstrate significant contextual influences on specific divisive topics.

==> unused/interpretation.tex <==
\section{Interpretation Case-Studies:  Climate Change, Gun Control, and Abortion}

\begin{figure*}[h!]
  \includegraphics[width=\textwidth]{odds_ratios.pdf}
  \caption{Odds ratios of the top and bottom 10 features in terms of influence. Labels for discourse acts are abbreviated as follows: \textit{question} $\rightarrow$ Q, \textit{answer} $\rightarrow$ A, \textit{announcement} $\rightarrow$ ANC, \textit{agreement} $\rightarrow$ AGR, \textit{appreciation} $\rightarrow$ APR, \textit{disagreement} $\rightarrow$ DGR, \textit{negative reaction} $\rightarrow$ NEG, \textit{elaboration} $\rightarrow$ ELB, \textit{humor} $\rightarrow$ HUM, \textit{other} $\rightarrow$ OTR, \textit{maximum selftext toxicity score} $\rightarrow$ max\_self\_tox, \textit{average comment polarity score} $\rightarrow$ avg\_com\_vad, \textit{maximum comment polarity score} $\rightarrow$ max\_com\_vad, \textit{average selftext polarity score} $\rightarrow$ avg\_self\_vad, \textit{maximum selftext polarity score} $\rightarrow$ max\_self\_vad, \textit{maximum comment toxicity score} $\rightarrow$ max\_com\_tox, \textit{minimum selftext polarity score} $\rightarrow$ min\_self\_vad, and \textit{title toxicity score} $\rightarrow$ title\_tox.}
  \label{fig:odds_ratios}
\end{figure*}

In this section, we will answer research questions 2(a) and 2(b) by examining the coefficients generated by the models trained in the predictive section. Explanations for the phenomena we observe in our data will be explained for each topic and the differences and similarities between topics will be investigated as well. We will use the coefficients generated by the TF-IDF + All model to interpret the decisions made by our models. We use the TF-IDF model instead of the BERT model for interpretation for better interpretability and robustness. Before interpreting them, we convert the coefficients into odds ratios for ease of interpretability. We will present hypotheses for the data overall and for each topic, and discuss whether or not the results confirm or deny these hypotheses and the implications of that information. The top $15$ odds ratios for each topic can be found in Figure~\ref{fig:odds_ratios}.

\subsection{Negative discourse acts are very informative, others are more complicated}
% Discourse features have been explored in controversy prediction work prior \cite{rethmeier-etal-2018-learning}, although these are lower-level features based on punctuation. While these are effective for prediction, they lack the inherent interpretability of higher-level discourse acts, especially by someone who is not versed in the field.

Discourse acts play an important role in all three topics and go a long way to helping answer RQ2a and b. The presence of negative discourse acts, in particular \textit{disagreement} and \textit{negative reaction}, are heavily indicative of controversy across all topics studied in this work. There are no instances where these two discourse acts have an odds ratio of less than one. This is unsurprising, as the manner in which participants react to conversations is heavily linked to how other participants perform discourse acts \cite{cramer2011controversy}. What is more surprising though, is the distribution of other discourse acts across other topics, and how negative discourse acts may "spoil" a conversation despite the presence of positive discourse acts like "appreciation" and "agreement". This is very easy to interpret and can be used by community or topic moderators with little training needed to pick out these negative discourse acts.

In climate change discourse acts of all kinds, expected and unexpected, are important features and integral to exploring what sorts of conversations are happening, especially when unexpected discourse acts are highly correlated with controversy, to better understand the nuances of these conversations. Looking at some examples of comments which fit these discourse patterns we can get a clearer picture of what is going on. The following posts follow the \textit{other}, \textit{agreement} pattern from a controversial conversation\footnote{The posts have been cut down for space. No content has been added.}:

\begin{displayquote}
\emph{...My guess is that a lot of this has come about because of the 'Climategate' hack, which seems to have convinced redditors that it's OK to abandon the scientific method when debating climate change... Can we kindly leave the politics and any crazy superstitions we might have in the appropriate subreddit and get back to the science?
Are there any actual scientists out there who feel the same way? 
Or is this just business as usual at /r/science?}

I agree. Most of the links posted here are blogspam, and the legitimate scientific papers get voted down. Alternatively, it might be worth it to start a start a new science reddit that is moderated by scientists. It's too easy for the deniers to vote good articles and comments out of existence on reddit.
\end{displayquote}

Which indicates that real discussion is going on, but not a particularly positive discussion in a thread that was concerning improperly posted climate skepticism related content. Or, for instance the following example of \textit{other}, \textit{agreement}:

\begin{displayquote}
Dear yanks
Enjoy your apocalypse. If it turns out like FO3, you're gonna have a blast.
Regards, 
Australia

Likewise, enjoy your Mad Max apocalypse down there!
\end{displayquote}

Which is an attempt at humor followed by sarcastic agreement. In any case, \textit{other} can mean anything from posts that are too long or short to be classified properly to nonsensical text. \textit{Agreement} does not mean positive conversation necessarily. The subject matter on which someone is agreeing can be extremely negative, as is demonstrated by the above examples. Since we focus our analyses on controversial topics, this may contribute to the importance attributed by our models to \textit{agreement} and other positive-seeming discourse acts.

\textit{Humor}, likewise, is worth exploring as a means of human expression that can be used both in lighthearted discussion and in less lighthearted insults and beratement.

\begin{displayquote}
Kind of like how congress mandated all bulbs become CFL's and theres no plan to dispose of them even though they contain poisonous levels of mercury.
Especially considering if a bulb breaks in your home the EPA recommends you evacuate all humans and pets and air out your house for at least 10 minutes for a single bulb

!!!! TEN MINUTES!?!??!!
\end{displayquote}

In which the second comment uses sarcastic humor to downplay the potential impact of broken CFL lightbulbs on human health. Contrast this with positive examples of humor:

\begin{displayquote}
Tell them it's a bad name for climate change.
What it means is more energy in the system, which in turn means more excitable weather. Hots get hotter, colds get colder, storms get larger and longer, climate belts shift around, earthquakes, volcanoes, the dead rising from the grave, dogs and cats living together... mass hysteria.

spit coke on the screen, damn you.
\end{displayquote}

Even \textit{appreciation}, the most overtly positive discourse act, does not strongly pull a conversation to be non-controversial on its own. This despite the fact that \textit{appreciation} appears more often than \textit{disagreement} and \textit{negative reaction} combined ($29,383$ vs. $18,012 + 10,534$). Indeed the intensities of these comments are captured in other features: the text representations themselves as well as toxicity features. Despite this weakness of the discourse features, \textit{negative reaction} and \textit{disagreement} remain powerful warning signs for controversy. This could be due to the negativity bias, which indicates that humans focus in more closely on negative information and have stronger physiological and psychological reactions to negative information. \cite{pratto1991automatic,soroka2019cross} Consider the following examples of \textit{disagreement}:

\begin{displayquote}
Oh that is exactly what happened. But they've been storing so much of their shit in my house, at no charge of course, that it literally took them an hour to pack it all up. They insulted me the entire time they were in MY home, packing up the things that had been taking up space in MY closet for months. I wanted them out IMMEDIATELY after I heard they had told my husband to leave me, they wouldn't get the fuck out. It just added to the unbelievable disrespect. They say awful things about me, tell my husband to leave me, insult me, and then act like they can take their sweet ass time getting out of my house. NO respect for me or the fact that it is my house whatsoever.
\end{displayquote}

\begin{displayquote}
But the ones I have met (i live in a rural-like area just at the city limits) are really agressive and racist. I find it pointless due to the fact that there is no need in this area...
\end{displayquote}

\begin{displayquote}
That logic doesn't work because having a baby doesn't invade a man's bodily autonomy.
\end{displayquote}

And now, \textit{negative reaction}:

\begin{displayquote}
Who the fuck downvotes this?
\end{displayquote}

\begin{displayquote}
I will say this: Most of this article is BULLSHIT. Collapsible stocks can go on 80\% of modern firearms. This is anti-gun propaganda, this article. 
\end{displayquote}

\begin{displayquote}
Haha, fuck off ;) I was neither hyperbolic or rude. "You're a terrible parent that should be jailed for killing your baby" That would be hyperbolic and rude. Go Fuck yourself. Cheers.
\end{displayquote}

These comments are all aggressive and inflammatory to varying degrees. Contrary to what one might expect, however, all of these examples are from non-controversial threads. The difference with these two discourse acts is that they appear five times as often in controversial threads, indicating that there may be a threshold before the negativity bias cannot be outmaneuvered by downvoting individual comments, or that negative comments appear too late in a thread's lifecycle in order to direct discourse significantly before the conversation dies down. It may also indicate that the toxicity of the thread and/or comments are spurring these reactions, the possibility of which will be investigated in a later subsection. This pattern, which manifests itself throughout all three topics studied here, indicates that high amounts of \textit{negative reaction} and \textit{disagreement} can indicate controversy and may warrant a moderator examining a thread for the more contextual clues that the other discourse acts require to fully understand RQ2.

\subsection{Controversiality can be connected to location in certain topics} User location can be very informative for certain topics, but not for others. In this section, we explore why that might be and discuss examples and implications of which locations appear in our data, which goes a long way to answer part of RQ2a and provides insight into RQ2b. User location is, as demonstrated by the coefficients, extremely variable in terms of both which features are represented and the importance of those features. Take, for instance, our model of the topic of climate change which highly values both California and New York, both of which are considered liberal states which are associated with the Democratic Party who, in turn, is generally associated with environmentalism. Contrast this with the model of the topic of gun control where users from locations generally associated with gun violence tragedies (e.g., Aurora, Colorado, USA) are considered heavily important, and thus the number of locations heavily weighted is higher. Further contrast both of these with abortion which tends to feature countries that are more open to the idea of abortion than the U.S. Despite the variance in location representation between topics these features offer an opportunity to study the differences between the reactions of users to content relating to specific events and the reactions of users to nonspecific, ongoing problems.

Our climate change model only heavily weighs a few location features. Of particular note are the locations California and New York, which are both heavily represented electorally by the Democratic party which is significantly more concerned about climate change on average than the Republican party\footnote{https://www.pewresearch.org/science/2015/07/01/chapter-2-climate-change-and-energy-issues/}. Those who are more concerned about the problem of climate change may, naturally, be more willing to argue for their position. Some examples of controversial threads in this category are as follows:

\begin{displayquote}
I believe that man made global warming to be made up, CMV

Americans, why does a lot of your population not "believe" in global warming?

Why are scientists so quick to point to man made climate change as the cause of hot temperatures when our temperature records are such a small sample size?
\end{displayquote}

Indeed, threads on these topics of climate change denial would draw the ire of those who are concerned about climate change, a large number of whom come from California and New York in the U.S. and may very likely downvote these threads, pushing them into our controversial category. In this case however, it isn't the discourse per se that is causing the controversy. These threads have significantly higher "answer" and "elaboration" discourse acts despite being controversial. However they also do often involve participants from the locations of New York and California. On the other side, threads that are directed to the attention of those that do not consider climate change a major issue tend to feature fewer relevant locations and more "disagreement" and "negative reaction" discourse acts. For instance, the thread:

\begin{displayquote}
Why does the Libertarian subreddit always feature climate change denial?
\end{displayquote}

Which, unexpectedly, was met with negative responses from unsatisfied users who may have felt antagonized by the original post.

Abortion falls into a similar place, where conversations about specific events with specific locations aren't uncommon as conversation topics but user locations do not tend to be as viscerally related to these topics. Two classes of location can be seen in the features for abortion: locations which are generally more accepting of abortion and locations which are generally less accepting of abortion. We see examples of the first category in \textit{in Germany}, \textit{DEU}, and \textit{in Britain} and examples of the second category in \textit{in Missouri} and \textit{in Texas}. The posts of these users, however, have very little to do with their place of residence, if anything at all. This could be indicative of a wide spread of people with complex views on abortion or on a diminished importance of particular locations.

Gun control presents a different view of location and controversy, one that is focused more on specific events and the locations where they took place. For instance, Aurora, Colorado where, in 2012, a shooting was carried out which killed 12 and injured 70\footnote{https://en.wikipedia.org/wiki/2012\_Aurora,\_Colorado\_shooting}. Many users that we have identified as being from the Denver area have participated in controversial threads specifically about the shooting. For instance, the following post posted on the news subreddit on July 20th, 2012, the morning after the event:

\begin{displayquote}
AURORA MASSACRE: THE COMPREHENSIVE TIMELINE

All information here has been independently gathered and aggregated. Accuracy, clarity, and transparency have been the main goals - but any postings (unless official police or hospital releases) should be taken at your own discretion.
\end{displayquote}

The rest of the post, which consists of a table filled with news reports, information, and links has been omitted. Humans tend to react to events spatially close to them more concretely and emotionally, \cite{fujita2006spatial} which may be what causes these conversations, along with the particularly volatile subject matter, to become controversial.
Contrast this with the topics of climate change and abortion where specific locations, although present, play a significantly smaller role in the overall discourse. They are both much broader issues that are less specific and temporally restricted than gun violence incidents.

Through our exploration of location features in our models we have determined that location is highly variable across topics as well as within them. In some topics, location may only play a broader role in controversy prediction, and the actual way in which language is used in conversation is more important as far as controversy is concerned. In other topics, locations may be extremely specific and related to similarly specific events. As such, detecting controversy in environments designed for very specific, spatially close locations can be viewed very differently from broader environments with more spatial separation. 

\subsection{Prolific users are more likely to participate in difficult conversations}
We hypothesized that high prolificity, the amount of users in a given thread who appear more than $x$ times in the dataset where $x \in \{25, 50, 100\}$, would be associated with lower levels of controversy and therefore help to answer RQ2a. However, this is not the case in our results. Although these features do still help us answer RQ2a, it is not accrding to expectations. In all three topics, the three prolificity features \textit{prolific\_25}, \textit{prolific\_50}, and \textit{prolific\_100} were associated at least slightly with controversy. It may be the reason for this is that prolific users are more likely to post in all threads, including controversial ones, whereas non-prolific users are less likely to comment on a thread that seems like it has gotten out of hand or will end up doing so. These users are not as comfortable in the online community as prolific users and, therefore, shy away from more difficult situations. Some examples, from the topic of abortion due to its high rating of prolificity, of highly prolific controversial thread titles are:

\begin{displayquote}
My girlfriend just got an abortion, AMA

I work at an abortion clinic. I put this up on our gate before a prayer vigil for 40 Days for Life. What does r/atheism think?

I have never spoken in depth about this, but am now ready. The horrors I endured while in a Catholic high school...seminary.

I became an atheist through being mocked as a theist.

It's true, hardcore assholes have set up fake abortion clinics, thousands of them, to mentally abuse women
\end{displayquote}

And non-controversial thread titles:

\begin{displayquote}
If you could see inside your womb, would you have an abortion? Why or why not?

Why are Christians so anti-abortion?

As a scientific mind, liberal, athiest, I'm having trouble with the issue of abortion. My friends hate me because of it. How do I deal with this?

From a lifelong Christian recently turned closet Atheist: Why it's never good to be honest with your conservative/religious Texan family.....
\end{displayquote}

There is a trend here, these prolific conversations tend to feature religious themes more often, regardless of controversy. Contrast that with low-prolificity controversial titlestitles:

\begin{displayquote}
Seemingly awesome guy asks me out, I find a massive dealbreaker in his match questions. Where do I go from here?

What reasons do you want to leave (WARNING PROBABLY OFFENSIVE TO SOME)?

Help me out with my college government class please!

GF doesn't want to have sex with me. Advices?

Men, would you date a young woman--22--who has an infant...by her dead ex-bf?

Women of reddit I have a weird question. Would you get an abortion on your birthday?
\end{displayquote}

And non-controversial thread titles:

\begin{displayquote}
My Take on Unwanted Pregnancies

I'm a product of rape, and I hate myself everyday for it. 

My son

And on a positive note:

Cleaning up the party platform
\end{displayquote}

We see significantly fewer religious themes emerging in these threads. We hypothesize that this religious element, among other things, dissuades newer, less prolific users from participating given the volatility conversations about religion can have.

\subsection{Gender and Gendered Topics}
Gender has an extremely variable impact on controversy depending heavily on whether or not gender is an inherent issue in whatever topic is being discussed, providing an answer to an important part of RQ2a. This is immediately evident in our analysis due to the fact that the presence of specific genders is only appreciably different when looking at abortion, with male having an odds ratio of $1.31$ compared to the female value of $1.11$. We hypothesize that the reason that female is still above $1$ is that controversial conversations tend to attract more participants, particularly online \cite{chen2013and}. Since we collect the number of participants who we can identify as a particular gender this means that higher numbers are generally associated with higher chance of controversy. The fact that gender can be so influential in the topic of abortion as to raise the odds ratio of male so high is a testament to the gender differences in controversial conversations \cite{herring2020dominates} and that abortion is a topic that particularly concerns women more than men. Those studying conversations in a particular community which may deal with female-centric issues more often than not may wish to heavily weigh gender as a feature of importance for determining controversy.

%\begin{comment}
\subsection{Toxic title lead to controversy, not toxic post}
Toxicity, as a signal for controversy detection, could have very different impact toward the prediction under different circumstances. \textit{Title toxicity} usually works well among all topics, despite these topics holding distinct overall toxic level. We hypothesize that toxic title itself could be viewed as click-bait, which will potentially attract people who refuse to participate calmly and gently, thus leading to a more controversial discussion. Other toxic features are performing differently among topics; If we take a deeper look at \textit{maximum comment toxicity}, which evaluate the extreme level of the toxicity for given conversations, we can observe that they are considered as useful only in abortion and gun control. This could be the case that different topic has different communities; people that involve in conversations under climate change topic tend to be less anti-social, making both controversial conversation as well controversial ones present low level of toxicity. We cannot verdict that toxicity always have a positive correlation with controversy. On the other hand, \textit{maximum selftext toxicity}, which present the extreme toxic level of given post, is contributing negatively in all topics. This is contradicting our instinct, as we think that the post is usually served as an expansion or explanation of the post title and provide context for people in the community, so that \textit{maximum selftext toxicity} should have similar weight in prediction as \textit{title toxicity}. One possible interpretation could be that in many cases people's attention tend to skip the detailed post and focus only on title and the conversations itself. Or things could be even simpler, that once people are attracted by the toxic title, they tend to stay in the conversations and contribute to the controversy, and only make use of the post itself as a reference to provide context.

\subsection{psychological analysis}
\begin{figure}[h!]
    \centering
    \includesvg[width=8cm]{LIWC_odds_selected.svg}
    \caption{Selected odd ratio for psychological features across topics.}
    \label{fig:odds_LIWC_selected.svg}
\end{figure}
Here we show analysis towards psychological features. The psychometrics of natural language use are not always useful, due to the nature of discourse that we don't usually repeat the same thing over and over again in a conversation~\cite{tausczik2010psychological}. In fact a large portion of the odds ratio from psychological features are close to $1$, but still there are a few categories that stand out from the others, which are shown in Table~\ref{fig:odds_LIWC_selected.svg}. Here we present the our analysis regarding the following features that really make a impact during prediction: \textit{You}, \textit{Friends} and \textit{Leisure}.
\subsubsection{You}
Feature \textit{You} stands for second-person pronouns, which generally refer to the person or persons being addressed. Some \textit{You} patterns are 'you', 'yall', 'youre', etc,. \textit{You} make positive contribution in predicting controversy for all topics. Though the contribution is relatively weak in some cases, the phenomenon is in line with our common sense: people that point at each other and blame each other are more likely to lead the discussion into argument. A example from climate change under this category is:
\begin{displayquote}
another thing "there's going to be some kind of hot bar" In an mmo? no fucking way please, enlighten us further

"The extent to which we can damage the environment is still unknown."

bullshit,if you have some info you have all of it

"That's under wraps pretty tight so I'd imagine its damageable to a good extent."

these are all just guesses
\end{displayquote}

In many cases the use of \textit{You} happen together with high toxicity context:
\begin{displayquote}
You're *literally* a neckbeard, eh?

Your little side note just suddenly made you sound like so many other self important, douchebag gamers who make the same kinds of claims. I've probably met a handful of people who think they somehow inspired some facet or system in gaming.

Pretty sure spell research goes back to tabletop gaming, so, you're from wizards or tsr, then? I hope you get your royalties for your contribution to fucking fantasy gaming.
\end{displayquote}
The examples shown explicitly reveal the intense relationship between the narrator and the target (to whom the word 'you' refer to). This phenomenon align with the finding by~\citeauthor{simmons2008hostile}, where they found that the use of second-person pronouns was negatively related to relationship quality.

\subsubsection{Friends}
The performance of \textit{Friends} patterns vary across topics. It has a positive influence while performing prediction on climate change, have almost no impact on gun control, and impact negatively on abortion. The category of \textit{Friends} includes patterns like 'bud', 'colleague', 'exgirl', 'exgirlfriend', etc,. This is categorized as content words in LIWC lexicon, which conveys the content of a communication~\cite{tausczik2010psychological}. It is more common that \textit{Friends} patterns show up in abortion topic that others, due to the fact that abortion topic is more individual-related, and people need to refer to these words while narrating in conversations. In fact, the average amount of usage for \textit{Friends} patterns in abortion is $26$, while the number is only $13$ in climate change, which demonstrate a bit of our assumption. The wide utilization of \textit{Friends} might make it harder to serve as a distinction signal in controversy prediction. We have a lot of comments like this in both controversial and non-controversial conversations in abortion:
\begin{displayquote}
My best friend had one and his relationship with his girlfriend didn't make it. I'm just telling you this to tell you that if you truly care for your girlfriend now is the time to show her. His ex said she felt like he cared about her if he wasn't willing to have a kid with her. I hope everything works out for the best for you, and I'm sure you made the right decision and I do support you. Good luck man
\end{displayquote}
and
\begin{displayquote}
If you weren't ready for a child then you're a jackass for not using protection (and your gf should've never agreed to unprotected sex), but I'm sure you both already know that and this has been a huge learning experience for you and your gf. That being said I hope you two make it through this alright, and never end up in this situation in the future. Hopefully many people reading this AMA will learn from the mistakes you and your gf made, 
so that this situation doesn't happen to anyone else either. What's done is done, best of luck in the future.
\end{displayquote}
In these examples \textit{Friends} patterns only serve the goal that either narrators can tell the full story clearly or narrators can make a sound argument. In both cases people need to refer to \textit{Friends} patterns so that making them seemly common in abortion. On the other hand, in climate change topic, the usage of \textit{Friends} behave kind of differently, like
\begin{displayquote}
Yeah I have friends going the same direction. Just be careful of where they send you or you might witness a surprise witch burning like a friend of 
mine did in Bolivia.
\end{displayquote}
or
\begin{displayquote}
If you got a girlfriend due to involvement in 4chan, you are definitely the exception not the rule. Also, there's a good chance your girlfriend used to be a dude.
\end{displayquote}
Here both examples are from threads which are considered controversy. We surmise that \textit{Friends} patterns are usually utilized in order to demonstrate a opinion or perform a sarcasm since they can provide a proper context or target. Here we present the top $3$ most used \textit{Friends} patterns for climate change as well as abortion in Table~\ref{table:wordcount}.

\begin{table}[h!]
\begin{center}
 \begin{tabular}{|l|p{2cm}|p{2cm}|}
\hline
\multirow{2}{*}{Topics} & \multicolumn{2}{c|}{Patterns} \\ \cline{2-3}
                        & \multicolumn{1}{l|}{\textit{Friends}} & \multicolumn{1}{l|}{\textit{Leisure}}                         \\\hline\hline
Abortion & \makecell[l]{friend*\\boyf*\\girlfriend*} & \makecell[l]{family\\party\\show} \\ \hline
Climate change & \makecell[l]{friend*\\neighbor*\\fellow*} & \makecell[l]{game\\play\\team} \\ \hline
Gun control  & \makecell[l]{friend*\\girlfriend*\\bf*} & \makecell[l]{game\\team\\play} \\ \hline
\end{tabular}
\caption{We list the top $3$ most used patterns for categories \textit{Friends} and \textit{Leisure} across all discussed topics.}
\label{table:wordcount}
\end{center}
\end{table}

From Table~\ref{table:wordcount} we can see that there is a distinct difference on the most frequently utilized words between the abortion and climate change, which could indicate their different use across topics. Also we observe a similar usage of \textit{Friends} patterns between abortion and gun control. This similarity could be the reason that \textit{Friends} could barely make any influence on controversy prediction with gun control topic, just like what \textit{Friends} does on abortion.

\subsubsection{Leisure}
\textit{Leisure} are the patterns that only make impact during the controversy prediction in climate change topic. \textit{Leisure} includes the patterns that people will directly refer to in order to reveal where individuals are focusing~\citep{tausczik2010psychological}, which contains patterns that indicate entertained behaviors or status such as 'bath', 'novel'. The relatively high weight of \textit{Leisure} seems contradict to our instinct since climate change has nothing to do with entertainments. We first take a glance at the most frequently used \textit{Leisure} patterns among topics. From \ref{table:wordcount} we find that the \textit{Leisure} pattern utilization on climate change and gun control are similar, indicating the content being video game, which is distinct from the most frequently used \textit{Leisure} patterns in abortion. Even though \textit{Leisure} are mostly referring to the same patterns in both climate change and gun control, their impact on controversy prediction differ greatly. In many cases in climate change we find that people are literally talking about games themselves, under a controversial situation, for example:
\begin{displayquote}
Honestly, while this might be marginally better, I would still be just as pissed off.  The entire reason I'm upset is that we went through 3 games (AC2,ACB,ACR) where Desmond is training to be a master assassin through the animus, then we get half an hour of gameplay in which he is demonstating 
his ability.  A better ending would have been, he touches the orb releasing Juno, and then is forced to chase her around the world where she has enthralled people to fight against you, the world has been saved from the solar flare, but now must be saved from mass enslavement. They could even have you play more as Connor making contact with Miranda, who would warn us of Juno's treachery and give us clues of how to stop her.
\end{displayquote}
In this example the participator complained about the plot development, which is definitely part of the game itself. Meanwhile from the examples extracted from gun control conversations, game is used for pushing the conversation forward and won't be the main content:
\begin{displayquote}
I'll share a friends missionary experience, since I doubt he'll ever join this forum.

He was on his mission in 1984 in Greensboro N. Carolina. He started the day off with a member of the ward going on a split with him, Bro. Card. A little bit into the day Bro. Card asks if they could go back to his apartment because he was expecting a package. My friend says sure, and they go back to his apartment where several boxes were waiting. They get all of the boxes inside and Bro. Card opens one up, picks up a copy of Ender's Game and says, "Here! This is for you!" So my friend has the first copy of Ender's Game touched by OSC. Yeah, Card is a scumbag, but I was unbelievably jealous of his experience and his copy of Ender's Game.
\end{displayquote}

We hypothesize that conversations which are directly related to games themselves could be controversial, while conversations that only have games to make points or convey messages will be harder to distinguish. While people talking about games themselves, including the commenting their quality or playability, their evaluations come from their own experience of the games, which could be subjective, and thus lead to controversy.


==> unused/old_psych.tex <==
Here we show analysis towards psychological features. The psychometrics of natural language use are not always useful, due to the nature of discourse that we don't usually repeat the same thing over and over again in a conversation~\cite{tausczik2010psychological}. In fact a large portion of the odds ratio from psychological features are close to $1$, but still there are a few categories that stand out from the others, which are shown in Table~\ref{fig:odds_LIWC_selected.svg}. Here we present the our analysis regarding the following features that really make a impact during prediction: \textit{You}, \textit{Friends} and \textit{Leisure}.
\subsubsection{You}
Feature \textit{You} stands for second-person pronouns, which generally refer to the person or persons being addressed. Some \textit{You} patterns are 'you', 'yall', 'youre', etc,. \textit{You} make positive contribution in predicting controversy for all topics. Though the contribution is relatively weak in some cases, the phenomenon is in line with our common sense: people that point at each other and blame each other are more likely to lead the discussion into argument. A example from climate change under this category is:
\begin{displayquote}
another thing "there's going to be some kind of hot bar" In an mmo? no fucking way please, enlighten us further

"The extent to which we can damage the environment is still unknown."

bullshit,if you have some info you have all of it

"That's under wraps pretty tight so I'd imagine its damageable to a good extent."

these are all just guesses
\end{displayquote}

In many cases the use of \textit{You} happen together with high toxicity context:
\begin{displayquote}
You're *literally* a neckbeard, eh?

Your little side note just suddenly made you sound like so many other self important, douchebag gamers who make the same kinds of claims. I've probably met a handful of people who think they somehow inspired some facet or system in gaming.

Pretty sure spell research goes back to tabletop gaming, so, you're from wizards or tsr, then? I hope you get your royalties for your contribution to fucking fantasy gaming.
\end{displayquote}
The examples shown explicitly reveal the intense relationship between the narrator and the target (to whom the word 'you' refer to). This phenomenon align with the finding by~\citeauthor{simmons2008hostile}, where they found that the use of second-person pronouns was negatively related to relationship quality.

\subsubsection{Friends}
The performance of \textit{Friends} patterns vary across topics. It has a positive influence while performing prediction on climate change, have almost no impact on gun control, and impact negatively on abortion. The category of \textit{Friends} includes patterns like 'bud', 'colleague', 'exgirl', 'exgirlfriend', etc,. This is categorized as content words in LIWC lexicon, which conveys the content of a communication~\cite{tausczik2010psychological}. It is more common that \textit{Friends} patterns show up in abortion topic that others, due to the fact that abortion topic is more individual-related, and people need to refer to these words while narrating in conversations. In fact, the average amount of usage for \textit{Friends} patterns in abortion is $26$, while the number is only $13$ in climate change, which demonstrate a bit of our assumption. The wide utilization of \textit{Friends} might make it harder to serve as a distinction signal in controversy prediction. We have a lot of comments like this in both controversial and non-controversial conversations in abortion:
\begin{displayquote}
My best friend had one and his relationship with his girlfriend didn't make it. I'm just telling you this to tell you that if you truly care for your girlfriend now is the time to show her. His ex said she felt like he cared about her if he wasn't willing to have a kid with her. I hope everything works out for the best for you, and I'm sure you made the right decision and I do support you. Good luck man
\end{displayquote}
and
\begin{displayquote}
If you weren't ready for a child then you're a jackass for not using protection (and your gf should've never agreed to unprotected sex), but I'm sure you both already know that and this has been a huge learning experience for you and your gf. That being said I hope you two make it through this alright, and never end up in this situation in the future. Hopefully many people reading this AMA will learn from the mistakes you and your gf made, 
so that this situation doesn't happen to anyone else either. What's done is done, best of luck in the future.
\end{displayquote}
In these examples \textit{Friends} patterns only serve the goal that either narrators can tell the full story clearly or narrators can make a sound argument. In both cases people need to refer to \textit{Friends} patterns so that making them seemly common in abortion. On the other hand, in climate change topic, the usage of \textit{Friends} behave kind of differently, like
\begin{displayquote}
Yeah I have friends going the same direction. Just be careful of where they send you or you might witness a surprise witch burning like a friend of 
mine did in Bolivia.
\end{displayquote}
or
\begin{displayquote}
If you got a girlfriend due to involvement in 4chan, you are definitely the exception not the rule. Also, there's a good chance your girlfriend used to be a dude.
\end{displayquote}
Here both examples are from threads which are considered controversial. We surmise that \textit{Friends} patterns are usually utilized in order to demonstrate a opinion or perform a sarcasm since they can provide a proper context or target. Here we present the top $3$ most used \textit{Friends} patterns for climate change as well as abortion in Table~\ref{table:wordcount}.

\begin{table}[h!]
\begin{center}
 \begin{tabular}{|l|p{2cm}|p{2cm}|}
\hline
\multirow{2}{*}{Topics} & \multicolumn{2}{c|}{Patterns} \\ \cline{2-3}
                        & \multicolumn{1}{l|}{\textit{Friends}} & \multicolumn{1}{l|}{\textit{Leisure}}                         \\\hline\hline
Abortion & \makecell[l]{friend*\\boyf*\\girlfriend*} & \makecell[l]{family\\party\\show} \\ \hline
Climate change & \makecell[l]{friend*\\neighbor*\\fellow*} & \makecell[l]{game\\play\\team} \\ \hline
Gun control  & \makecell[l]{friend*\\girlfriend*\\bf*} & \makecell[l]{game\\team\\play} \\ \hline
\end{tabular}
\caption{We list the top $3$ most used patterns for categories \textit{Friends} and \textit{Leisure} across all discussed topics.}
\label{table:wordcount}
\end{center}
\end{table}

From Table~\ref{table:wordcount} we can see that there is a distinct difference on the most frequently utilized words between the abortion and climate change, which could indicate their different use across topics. Also we observe a similar usage of \textit{Friends} patterns between abortion and gun control. This similarity could be the reason that \textit{Friends} could barely make any influence on controversy prediction with gun control topic, just like what \textit{Friends} does on abortion.

\subsubsection{Leisure}
\textit{Leisure} are the patterns that only make impact during the controversy prediction in climate change topic. \textit{Leisure} includes the patterns that people will directly refer to in order to reveal where individuals are focusing~\citep{tausczik2010psychological}, which contains patterns that indicate entertained behaviors or status such as 'bath', 'novel'. The relatively high weight of \textit{Leisure} seems contradict to our instinct since climate change has nothing to do with entertainments. We first take a glance at the most frequently used \textit{Leisure} patterns among topics. From \ref{table:wordcount} we find that the \textit{Leisure} pattern utilization on climate change and gun control are similar, indicating the content being video game, which is distinct from the most frequently used \textit{Leisure} patterns in abortion. Even though \textit{Leisure} are mostly referring to the same patterns in both climate change and gun control, their impact on controversy prediction differ greatly. In many cases in climate change we find that people are literally talking about games themselves, under a controversial situation, for example:
\begin{displayquote}
Honestly, while this might be marginally better, I would still be just as pissed off.  The entire reason I'm upset is that we went through 3 games (AC2,ACB,ACR) where Desmond is training to be a master assassin through the animus, then we get half an hour of gameplay in which he is demonstating 
his ability.  A better ending would have been, he touches the orb releasing Juno, and then is forced to chase her around the world where she has enthralled people to fight against you, the world has been saved from the solar flare, but now must be saved from mass enslavement. They could even have you play more as Connor making contact with Miranda, who would warn us of Juno's treachery and give us clues of how to stop her.
\end{displayquote}
In this example the participator complained about the plot development, which is definitely part of the game itself. Meanwhile from the examples extracted from gun control conversations, game is used for pushing the conversation forward and won't be the main content:
\begin{displayquote}
I'll share a friends missionary experience, since I doubt he'll ever join this forum.

He was on his mission in 1984 in Greensboro N. Carolina. He started the day off with a member of the ward going on a split with him, Bro. Card. A little bit into the day Bro. Card asks if they could go back to his apartment because he was expecting a package. My friend says sure, and they go back to his apartment where several boxes were waiting. They get all of the boxes inside and Bro. Card opens one up, picks up a copy of Ender's Game and says, "Here! This is for you!" So my friend has the first copy of Ender's Game touched by OSC. Yeah, Card is a scumbag, but I was unbelievably jealous of his experience and his copy of Ender's Game.
\end{displayquote}

We hypothesize that conversations which are directly related to games themselves could be controversial, while conversations that only have games to make points or convey messages will be harder to distinguish. While people talking about games themselves, including the commenting their quality or playability, their evaluations come from their own experience of the games, which could be subjective, and thus lead to controversy.

